Learning from Imperfect Human Feedback: a Tale from Corruption-Robust Dueling

This paper studies Learning from Imperfect Human Feedback (LIHF), addressing the potential irrationality or imperfect perception when learning from comparative human feedback. Building on evidences that human's imperfection decays over time (i.e., humans learn to improve), we cast this problem as a concave-utility continuous-action dueling bandit but under a restricted form of corruption: i.e., the corruption scale is decaying over time as $t^{\rho-1}$ for some "imperfection rate" $\rho \in [0, 1]$. With $T$ as the total number of iterations, we establish a regret lower bound of $ \Omega(\max\{\sqrt{T}, T^{\rho}\}) $ for LIHF, even when $\rho$ is known. For the same setting, we develop the Robustified Stochastic Mirror Descent for Imperfect Dueling (RoSMID) algorithm, which achieves nearly optimal regret $\tilde{\mathcal{O}}(\max\{\sqrt{T}, T^{\rho}\})$. Core to our analysis is a novel framework for analyzing gradient-based algorithms for dueling bandit under corruption, and we demonstrate its general applicability by showing how this framework can be easily applied to obtain corruption-robust guarantees for other popular gradient-based dueling bandit algorithms. Our theoretical results are validated by extensive experiments.

==> 0-abstract.tex <==
\begin{abstract}
This paper studies Learning from \emph{Imperfect} Human Feedback (LIHF), motivated by humans' potential  irrationality or imperfect perception of true preference. We revisit the  classic dueling bandit problem as a model of learning from comparative human feedback, and enrich it by casting the imperfection in human feedback as \emph{agnostic} corruption to user utilities. We start by identifying the fundamental limits  of LIHF and prove a regret lower bound of $\Omega(\max\{T^{1/2},C\})$, even when the total corruption $C$ is known and when the corruption decays gracefully over time (i.e.,  user feedback becomes increasingly more accurate). We then turn to design robust algorithms applicable in real-world scenarios with arbitrary corruption and unknown $C$. Our key finding is that gradient-based algorithms enjoy a smooth efficiency-robustness tradeoff under corruption by varying their learning rates. Specifically, under general concave user utility, Dueling Bandit Gradient Descent (DBGD) of \cite{Yue2009InteractivelyOI} can be tuned to achieve regret $O(T^{1-\alpha} + T^{ \alpha} C)$ for any given parameter $\alpha \in (0, \frac{1}{4}]$. Additionally, this result enables us to pin down the regret lower bound of the standard DBGD (the $\alpha=1/4$ case) as $\Omega(T^{3/4})$ for the first time, to the best of our knowledge. For strongly concave user utility we show a better tradeoff: there is an algorithm that achieves $O(T^{\alpha} + T^{\frac{1}{2}(1-\alpha)}C)$ for any given $\alpha \in [\frac{1}{2},1)$. Our theoretical insights are corroborated by extensive experiments on real-world recommendation data.  
\end{abstract}

==> 1-introduction.tex <==
\section{Introduction}
Many real-world problems, such as personalized recommendation \citep{Yue2009InteractivelyOI, immorlica2020incentivizing,yao2022learning} and fine-tuning generative models \citep{bai2022training,casper2023open, han2024parameterefficient}, require learning from human feedback. Expressing preferences as numerical values or concrete functions is generally challenging for humans. Therefore, an approach that has achieved significant real-world success is to learn humans' preferences by eliciting their comparative feedback between two options \citep{bai2022training}. A natural theoretical framework capturing such learning task is the seminal dueling bandits framework introduced by \cite{Yue2009InteractivelyOI}. The dueling bandit problem features an sequential online learning problem, during which a pair of actions are selected at each round and only their comparison result is revealed to the learner. The comparison outcome between two actions is modeled using a utility function of actions, alongside a link function that determines the probability of each action winning based on their utility difference. This modeling approach is termed as utility-based dueling bandit and achieves great success in generating summaries closely aligned with human preferences \citep{stiennon2020learning}. 

However, human feedback is often \emph{imperfect}, a crucial factor that has been largely overlooked in previous studies of  dueling bandit. Ample  behavioral studies show that humans often refine their preferences through interactions with the system, navigating a complex tradeoff between exploration and exploitation \citep{wilson2014humans, cohen2007should}. Furthermore, their response errors may exhibit systematic patterns rather than merely random noise.  As we are all aware of, humans are not always rational \citep{posner1997rational} neither perfectly know our preferences \citep{pu2012evaluating}. 

In this paper, we study learning from \emph{imperfect} human feedback (LIHF) by casting the imperfection in the feedback as certain form of corruption to the utilities. This leads us to study a natural variant of the continuous dueling bandit with corrupted utilities. Notably, our study differs from recent robust algorithms designed for corrupted dueling bandits \citep{di2024nearly, pmlr-v162-saha22a, komiyama2015regret} in three key aspects. Firstly, these previous algorithms all focus on a finite action space whereas, to the best of our knowledge, ours is the first to investigate a robust dueling bandit algorithm under corruption for continuous action space. This focus is motivated by the fact that many real-world applications have continuous or extremely dense action spaces, such as token embeddings or content recommendations \citep{chen2021decision, chen2019large}.  Second, our algorithms are designed for \emph{agnostic} corruption without knowing the corruption levels, whereas \cite{di2024nearly} requires knowledge of the total corruption amount. This focus on agnostic corruption is motivated by realistic considerations, because systems often cannot accurately discern the irrational or imperfect nature of human feedback. Third, our corruption models are very different from the model studied by \cite{di2024nearly, pmlr-v162-saha22a, komiyama2015regret}. The  corruption in their model contaminates feedback by flipping the realized outcomes of the duels, whereas the corruption in our model is on utilities which consequently only alter the winning probabilities of the duels. This difference is due to our different motivation of corruption, which is to capture imperfect human behavior while not intentional adversarial attack (see more illustration in Section \ref{sec:model}).

\vspace{10pt}
\noindent \textbf{Our Contributions.} By modeling LIHF as a continuous dueling bandit under agnostic corruption, we start by characterizing its intrinsic hardness. We prove a regret lower bound of $\Omega(d\max\{\sqrt{T}, C\})$, even when the total corruption $C$ is known and when corruption decays gradually over time. Additionally, we prove that this lower bound result is tight by exhibiting an algorithm that indeed achieves a matching upper bound for the aforementioned setting. Next, we turn to design robust algorithms that are applicable to  arbitrary and agnostic corruption with unknown $C$. Our key finding is that gradient-based algorithms offer a smooth efficiency-robustness tradeoff under corruption by carefully tuning their learning rates. Specifically, let $d$ denote the problem dimension. For any given $\alpha \in (0, 1/4]$,  Dueling Bandit Gradient Descent (DBGD) \citep{Yue2009InteractivelyOI} with carefully chosen learning rate (that depends on $\alpha$) can achieve a regret of $O(\sqrt{d}T^{1-\alpha} + \sqrt{d}T^{\alpha}C)$ under arbitrary concave user utility. That is, by decreasing $\alpha$ from $1/4$ to $0$, the regret under no corruption (i.e., learning efficiency) decays from $\sqrt{d}T^{3/4}$ to $\sqrt{d}T$  but the algorithm's tolerance to total amount of corruption   increases from $O(T^{3/4})$ to $O(T)$ (i.e., more robustness). Perhaps surprisingly, this result turns out to allow us to pin down a regret lower bound for the standard version of DBGD (the $\alpha=1/4$ case) as $\Omega(T^{3/4})$, marking the first tight lower bound result for the DBGD algorithm to the best of our knowledge. For strongly concave user utility, we show that an improved tradeoff is possible: Noisy Comparison based Stochastic Mirror Descent (NC-SMD) \citep{kumagai2017regret} can be refined to achieve a regret of $O(dT^{\alpha} + \sqrt{d}T^{\frac{1-\alpha}{2}}C + dC)$ for any given $\alpha \in [1/2, 1)$. We remark that similar robustness-accuracy tradeoff has been  studied classification problem with adversarial examples, both  empirically \citep{tsipras2018robustness} and theoretically \citep{zhang2019theoretically}. However, to the best of our knowledge, this is the first time such tradeoff is formally analyzed for online learning. Finally, we conduct extensive experiments on real-world recommendation data to validate our theoretical insights.


\section{Related Work}
\textbf{Hardness of Learning from Imperfect Human Feedback}: To design algorithms robust to adversarial corruption, it is crucial to understand the intrinsic hardness of learning from corrupted feedback. \cite{lattimore_szepesvári_2020} demonstrates that the minimax regret lower bound for stochastic linear bandits is $\Omega(d\sqrt{T})$. Utilizing the regret lower bound for bandit convex optimization \citep{shamir2013complexity}, \cite{kumagai2017regret} illustrates that dueling bandits with a strongly concave utility function achieve a regret lower bound of $\Omega(d\sqrt{T})$. In scenarios of adversarial corruption, \cite{bogunovic2020stochastic} proves that any algorithm faces regret at least $\Omega(dC)$ for stochastic linear bandits. However, currently there is no literature that has explored the intrinsic hardness of learning from corruption which decays gradually over time \citep{wilson2014humans, kumagai2017regret, cohen2007should}, despite its prevalence in learning from imperfect human feedback. 
% For example, as users interact with a recommendation system, their feedback tends to become more and more accurate, since the user gradually learns her preference \citep{wilson2014humans, kumagai2017regret, cohen2007should}. 
It still remains unknown whether learning from such corruption is fundamentally easier than learning from arbitrary corruption.

\vspace{10pt}
\noindent  \textbf{Stochastic Bandits with Unknown Corruption}: Applying the principle of optimism in face of uncertainty and constructing estimators involving uncertainty weighting, algorithms devised by \cite{he2022nearly} and \cite{ye2024robust} attain nearly optimal regret bounds for both linear and nonlinear contextual bandits in presence of adversarial corruption. By leveraging the concept of phase elimination, \cite{bogunovic2022robust} introduces a robust algorithm capable of handling corruption in rewards drawn from Gaussian processes. However, the designs of these algorithms require explicit knowledge of the total corruption level $C$ as an input. \cite{pmlr-v99-gupta19a} employ novel sampling strategy to channel resources to arms with better performance and craft algorithms robust to agnostic corruption, yet restricted to finite action sets. In scenarios involving continuous action set with unknown corruption level, even though algorithms designed by \cite{pmlr-v151-ding22c} and \cite{bogunovic2020stochastic} have sublinear regret guarantee, the regret is at least $C$ times worse than the regret without corruption. It remains as an open problem of whether better regret guarantee is achievable---that is, affording unknown corruption level more than $\Omega(\sqrt{T})$ while maintaining $O(\sqrt{T})$ regret guarantee in scenario without corruption.

\vspace{10pt}
\noindent \textbf{Continuous Dueling Bandits with Unknown Corruption}: In addition to stochastic bandits, there exists an extensive body of literature studying the dueling bandit problem with unknown corruption, given its prevalence in real-world application \citep{bengs2021preferencebased, sui2018advancements}. The literature on dueling bandits with adversarial corruption has been initially explored by \cite{pmlr-v132-agarwal21a} and subsequently enhanced by \cite{pmlr-v162-saha22a}, which achieves optimality in term of $C$. However, their work is solely applicable to finite action sets, which may not be feasible in many real-world scenarios that have continuous or extremely dense action spaces, such as token embeddings or content recommendations \citep{chen2021decision, chen2019large}. \cite{ailon2014reducing} introduced a reduction method that translates existing results from conventional Multi-Armed Bandit algorithms to Dueling Bandits. This reduction method is applicable to both finite and continuous action spaces, albeit requiring a linear link function. DBGD \citep{Yue2009InteractivelyOI} and NC-SMD \citep{kumagai2017regret} enjoy flexibility in choosing the link function but only work for continuous dueling bandits. It still remains as an open problem for developing provably efficient algorithm capable of learning from corrupted dueling feedback with unknown corruption in continuous action space. This serves as the driving force behind our theoretical analysis. 

 






==> 2-model.tex <==
\section{The Problem of Learning from Imperfect Human Feedback (LIHF)}\label{sec:model}
\textbf{Conventional Notation.} Throughout the paper, for a positive integer $T$, we use $[T]$ to denote $\{1, 2, \ldots, T\}$. We use $\cP_{\cA}(a)$ to denote the projection of action $a$ on $\cA$. We use standard asymptotic notations including $O(\cdot)$, $\Omega(\cdot)$, $\Theta(\cdot)$. We use $\Tilde{O}(\cdot)$, $\Tilde{\Omega}(\cdot)$, $\Tilde{\Theta}(\cdot)$ to hide logarithmic factors. We use $\|\cdot\|_{\infty}$ to define infinity norm. $\text{Reg}_T$ represents regret with dueling feedback over $T$ rounds.

To capture learning from imperfect (comparative) human feedback, we now introduce a natural variant of the seminal dueling bandit framework \citep{Yue2009InteractivelyOI} by integrating the ``imperfections'' in human feedback as certain corruption to human agents' feedback. An immediate critique one might have is that arbitrarily adversarial corruption seems too pessimistic as a way to model humans' inaccuracies which are often caused by uncertainty or ignorance, rather than targeted attacks. While this may appear true at the first glance,  we provide strong theoretical and empirical evidences that corruption caused by uncertainties generally is as hard as arbitrary corruption. For such reasons,  we coin the following problem \emph{Learning from Imperfect Human Feedback} (LIHF).

\vspace{10pt} 
\noindent \textbf{Basics of Dueling Bandits and Assumptions.} We consider the standard dueling bandit framework with continuous \emph{action} set $\mathcal{A} \subset \mathbb{R}^d$ \citep{Yue2009InteractivelyOI}. At each round $t\in[T]$, the learner (henceforth denoted as $\mathcal{L}$) chooses two actions $a_t, a'_t$ to present to some human agent, henceforth denoted as  the ``user''. The user receives \emph{utility} $\mu(a_t), \mu(a'_t)$ from the two actions respectively, and will pick one of these actions following a \emph{link} function $\sigma(\cdot)$. That is, in absence of any corruption, the user picks action $a_t$ with probability $\sigma(\mu(a_t) - \mu(a'_t))$, and action $a'_t$ otherwise. As clear from its definition, this choice probability depends only on the utility difference $\mu(a_t) - \mu(a'_t)$.  Notably, user's randomized action does carry information about underlying utility function $\mu$, which is why the action is also called the ``human feedback'' \citep{bengs2021preference, maystre2017just, ailon2014reducing}. Following standard assumptions in this literature \citep{kumagai2017regret, Yue2009InteractivelyOI}, we also assume
\begin{enumerate}[leftmargin=15pt]
    \item the continuous action space $\cA$ contains the origin, is compact, convex and is contained in a $d$-dimensional ball of radius $R$; 
    \item the utility function  $\mu: \cA \rightarrow \bR$ is concave, differentiable, $L_{\mu}$-Lipschitz and admits unique optimal within set $\cA$, denoted as $a^{*} := \arg \max_{a \in \cA} \mu(a)$;
    \item the link function $\sigma: \bR \rightarrow [0, 1]$ is rotational-symmetric, $L_{\sigma}$-Lipschitz and its first derivative $\sigma'$ is $L_2$-Lipschitz. 
\end{enumerate} 
For convenience, we further let $L = L_{\sigma}L_\mu$. Notably, some previous works restrict link function to specifically be the logistic link function \citep{di2024nearly, xu2024principled, saha2021optimal}. However, our results shall be applicable to any link functions that satisfy the natural assumptions above.  

\vspace{10pt}
\noindent \textbf{Inaccuracies in Human Feedback as Agnostic Corruption.} Extending the standard dueling bandit framework above, we introduce a \emph{corruption} term $c_t(a_t, a'_t)$ to the utility difference in order to model potential inaccuracy in the user's perception of underlying true utilities. For all our positive results, we always work with the situation where this corruption is \emph{agnostic} in the sense that the learner does not know the value of each $c_t$ neither their accumulated sum. Such agnostic corruption is natural because in reality it is very difficult to truly estimate how imperfect a user is, hence we aim to develop algorithms whose execution is agnostic to such parameters.  Let $a \succ a'$ denote the event that the user chooses $a$  over $a'$. Hence in our LIHF problem, the probability of event $a \succ a'$ in presence of corruption  $c(a, a')$, denoted as $\hat \bP(a \succ a') $, can be expressed as follows $ \hat \bP(a \succ a')  = \sigma(\mu(a) - \mu(a') + c(a, a'))$. We further let $\hat\cF(a_t, a'_t)$ denote user's preferential feedback under corruption, coined \textit{corrupted dueling feedback}. Mathematically, $\hat \cF(a_t, a'_t)$ follows a binomial distribution with mean $\hat \bP(a_t \succ a'_t)$, expressed by the following equation.
\begin{equation*}\label{equation:corrupted feedback}
        \hat \cF(a_t, a'_t):= \begin{cases}
        1 \hspace{1mm} \text{w.p.} \hspace{1mm} \hat \bP(a_t \succ a'_t)\\
        0 \hspace{1mm} \text{w.p.} \hspace{1mm} 1- \hat \bP(a_t \succ a'_t)
    \end{cases}
\end{equation*}

The ``hat'' notation in $\hat \cF$ and $\hat \bP $ is to denote corruption. When there is no corruption, we use $\mathbb{P}(a \succ a') = \sigma(\mu(a) - \mu(a') ) $ to denote the probability of event $a \succ a'$ and $\mathcal{F}(a, a')$ to denote corresponding dueling feedback. It is important to recognize the different roles of the link function $\sigma$ and utility corruption $c_t$ --- $\sigma$ captures the inherent (often inevitable) randomness in human choice/behavior even given true utilities \citep{fishburn1979utility,becker1963stochastic, bradley1952rank}, whereas our $c_t$ is introduced to model inaccurate perception of utilities due to not perfectly knowing her preferences and, importantly, can be alleviated or even eliminated once the user has tried sufficient actions. 

Imperfect user feedback generally is not as wild as arbitrary adversarial corruption. A particularly natural pattern of human's imperfection is that the inaccuracy in our estimations often diminishes as we try more and more actions. That is, humans learn along the way, though how fast the inaccuracy decreases often depends on our learning rate. This hence motivates us to consider the following notion of  $\rho$\emph{-imperfect user} which  significantly constrain the corruption sequence $c_1, c_2, \cdots $, and force it to diminish at the rate $\rho$. 

\begin{definition}[$\rho$-Imperfect User]\label{def:general-adversary}
The user feedback is said to be $\rho$-imperfect for some $\rho \in [0, 1]$  if there exists a constant $C_\kappa > 0$ such that the corruption  $c_t$ satisfies  $ |c_t| \leq C_\kappa t^{ \rho - 1}, \forall t \in [T]$.\footnote{All our results naturally applies to $\rho < 0$, which is  a significantly easier situation since accumulated corruption is a constant in that case. We hence will not explicitly consider it in this paper. }
\end{definition}

For a $\rho$-imperfect user, the accumulated corruption $\sum_{\tau = 1}^{t-1} |c_\tau| \leq C_\kappa t^{ \rho} $ for every $t$, which is why this is coined $\rho$-imperfect. The diminishing inaccuracy of user estimation in Definition \ref{def:general-adversary} is a natural model for user's learning behavior and  has already been used in various previous works to model user's imperfect feedback \citep{wang2023followups, yao2022learning, immorlica2020incentivizing} (Details are presented at Appendix \ref{sec:appendix_A}). Note that agnostic corruption in this situation means the learner know $ |c_t| \leq C_\kappa t^{ \rho - 1}$ for some $\rho$, but she does not know the value of $\rho$. 

On the other hand, the corruption are said to be \emph{arbitrary} up to certain budget  $C$,  if  $\sum_{t = 1}^{T} |c_t| \leq C$ for a given (hence fixed) time horizon $T$. Our designed (positive) learning algorithmic will have guaranteed regret upper bound under  arbitrary corruption, though our lower bound (i.e., negative result) will hold even in the weaker $\rho$-imperfect user feedback.

We remark that another line of recent research studies a different type of corruption that directly flip the outcomes of the duels; i.e., flipping the realized event $a \succ a'$ to its opposite $a' \succ a$ \citep{di2024nearly, pmlr-v162-saha22a, komiyama2015regret}. These corruption models are motivated by the existence of   true \emph{adversaries}, e.g., malicious users in recommendation systems \citep{lykouris2018stochastic} or fraudulent clicks \citep{deshpande2013linear}, who have the capability of altering user choices. In contrast,  only utilities are corrupted in our model. These two models are not comparable. For instance, the adversary can induce a deterministic event $a \succ a'$ at any given round with one corruption, whereas the outcomes in our model is almost always probabilistic (unless the adversary uses an infinite budget $c_t$). Such modeling difference inherently comes from the different motivations of our LIHF problem. Specifically, our model is to capture imperfect human feedback due to inaccurate perception of utilities or ignorance of true preferences.  For example, when recommender systems learn to find the optimal recommendation for a user, the user may not know her true preference at the beginning and often gradually refines her preferences through experiencing different items \citep{yao2022learning2}. Similarly, when generative models like ChatGPT learn to generate personalized content for a user, the user may go through a similar procedure of preference refinement during interactions with the model. These modelling differences also necessitate our fundamentally different techniques. Our approaches are based on gradient-based methods whereas \cite{di2024nearly} and \cite{saha2021optimal} employ the principle of optimistic in face of uncertainty and construct the confidence set of preferences through querying the maximum information pair. Their approaches inherently  require the knowledge of total corruption level $C$. In contrast, the analysis of our gradient-based methods controls the impact of  gradient bias (due to corruption) on regret. By adjusting its learning rate,  our algorithm will gracefully ``trade'' its learning efficiency for more robustness against agnostic corruption. Moreover,  our algorithm is suitable for infinite \emph{action} space, whereas previous works of \cite{di2024nearly,saha2021optimal} are for finite action spaces.

\vspace{10pt}
\noindent \textbf{Learning goal: agnostic corruption-robust regret minimization. } The goal of the learner is to optimize her sequential actions to minimize the following dueling regret against an arbitrary sequence of corruption $\{c_t\}_{t=1}^T$: 
\begin{equation}\label{def:DB_reg}
    \text{Reg}_T = \bE\left(\sum^T_{t=1}\sigma(\mu(a^*)-\mu(a_t)) + \sigma( \mu(a^*) - \mu(a'_t))-1\right).
\end{equation}
This regret measure is also studied in many prior literature \citep{pmlr-v162-saha22a, kumagai2017regret, komiyama2015regret, Yue2009InteractivelyOI}.
Importantly, all our algorithms are agnostic to the corruption in the sense that the algorithm does \emph{not} depend on any knowledge of $\{c_t\}_{t=1}^T$.  




==> 3-lower-bound.tex <==
\section{The Intrinsic Limit of Learning from Imperfect Human Feedback}\label{sec:lower-bound}
To understand the inherent difficulty of LIHF, in this section we develop regret lower bounds for a setting that is even easier to learn -- that is, learning from a $\rho$-imperfect user (Definition \ref{def:general-adversary}) with a \emph{known} $\rho$. While this non-agnostic may appear simpler, our main result of this section exhibits a tight lower bound of $\Omega (d\max\{\sqrt{T}, T^{\rho}\})$ for strongly concave user utilities.
% \footnote{$\Tilde{\Theta}$ ignores logrithmic terms.} 
We also show a similar lower bound hold for linear user utility as well. Our lower bound result differs in two key aspects from  various previous lower bound results for online learning under corruptions \citep{pmlr-v132-agarwal21a, bogunovic2020stochastic}. Firstly, previous lower bound proofs require the adversaries' capability to corrupt the reward feedback in an \emph{arbitrary} way, whereas the corruption in our proof will follow Definition \ref{def:general-adversary}. It is unclear whether such  strictly more restrictive corruption will be more tractable since it does offer the learner much more accurate estimation about the amount of corruption  at each round. Secondly, previous construction of hard instances that attains regret lower bound relies on  linear reward, whereas our lower bound holds for strongly concave utility functions, since they more realistically model human's risk attitude and consumption utilities \citep{1ac45b27-6b89-3b45-adcb-77e093f1ef0a}. Strongly concave utility functions are generally perceived as easier to optimize and to learn, hence it is unclear whether it is also the case under imperfect user feedback. While both differences above seem to hint that our problem might be easier than previous online learning problem under corruption, we show that the answer is actually ``No''.  

\begin{theorem}[A Tight Lower Bound]\label{theorem:regret_lower_bound}
There exists an LIHF instance with a $\rho$-imperfect user (Def. \ref{def:general-adversary}) and strongly concave user utility such that any learner  has to suffer $\text{Reg}_T \geq \Omega(d\max\{\sqrt{T}, T^{\rho}\})$ even \emph{with the knowledge of} $\rho$. Moreover, this regret lower bound is tight, up to logarithmic terms. That is, for the same setting, there exists an online learning algorithm with $\text{Reg}_T \leq \Tilde{O}(d\max\{\sqrt{T}, T^\rho\})$. 
\end{theorem}

This theorem  reveals the fundamental limits of learning from $\rho$-imperfect users, even when the learner knows $\rho$. The core new lemma needed for proving the regret lower bound in Theorem \ref{theorem:regret_lower_bound} is to show that even in standard online learning with noisy bandit feedback about any pulled arm's reward (as opposed to comparative feedback in dueling setups), the same regret lower bound holds. This is summarized in the following Lemma \ref{lemma:lower bound}. We then convert this lower bound for standard bandit reward feedback to our setting of dueling/comparative feedback. Notably,  \cite{ye2024corruptionrobust} recently showed a matching upper bound for the standard bandit reward feedback setting assuming \emph{arbitrary corruption} with total amount $C$. Hence Lemma \ref{lemma:lower bound} and their results together echoes our key insight in this section --- that is, learning from $\rho$-imperfect user is  as hard as learning from arbitrarily corrupted rewards in classic bandit reward feedback setting as well.   

For linear user utility, perhaps unsurprisingly, we are able to show the same lower bound as follows (see Prop. \ref{prop:regret_lower_bound_linear}). En route, we similarly show that the problem of learning directly from bandit linear reward feedback also suffers the same regret lower bound $\Omega(d\max\{\sqrt{T}, T^{\rho}\})$. This happens to resolve an open problem proposed by \citet{yao2022learning} and implies that the regret upper bound shown in \citep{yao2022learning} for the ``learning from learning user'' problem is tight in $T$. 

\begin{proposition}\label{prop:regret_lower_bound_linear}
There exists an LIHF instance with a $\rho$-imperfect user and linear user utility  such that any learner knowing $\rho$  has to suffer $\text{Reg}_T \geq \Omega(d\max\{\sqrt{T}, T^{\rho}\})$. 
\end{proposition}

We defer the full proof of Theorem \ref{theorem:regret_lower_bound} and Proposition \ref{prop:regret_lower_bound_linear} to Appendix \ref{proof:theorem:regret_lower_bound} and \ref{proof:lemma:linear_regret_lower_bound}. Below we only state a representative core lemma for the strongly concave utility function case and its proof sketch, which is the crux of our lower bound proof. Notably, the proof for the matching upper bound in Theorem \ref{theorem:regret_lower_bound} is also highly non-trivial. Our starting point is the recent NC-SMD algorithm. However, to achieve the tight regret upper bound, we have to employ a novel and highly involved induction argument to identify the optimal learning rate. Through this process, we  established a new connection between the convergence of the $L_2$-norm of the action $\|a_t - a^*\|_2$ and the regret itself (It has been experimentally verified at Appendix \ref{sec:known}).

\begin{lemma}\label{lemma:lower bound}
    Assume that the action space $\cA$ is contained in a $d$-dimensional unit ball. Consider the utility function $\mu$ in the form $\mu_{\theta}(a) = \theta^{\top}a - \frac{1}{2}\|a\|^2_2$, where $\theta \in \bR^d, \|\theta\|_2 \leq 1$, is a random vector. Under corruption induced by $\rho$-\emph{imperfect} user (Def. \ref{def:general-adversary}), for any fixed number of rounds $T$ and $d \leq \frac{1}{C_{\kappa}}T^{1-\rho}$, there exists a preference parameter $\theta$ such that for any learner $\cL$ under reward feedback, \emph{even with the knowledge of $\rho$}, has to suffer regret
    $\text{Reg}_T := \bE\{\sum^T_{t=1} \mu_{\theta}(a^*) - \mu_{\theta}(a_t)\} \geq \frac{d}{4}C_{\kappa}T^{\rho}.$
\end{lemma} 
\begin{proof}\textbf{(Proof Sketch of Lemma \ref{lemma:lower bound}).} 
We aim to show that there exists a corruption strategy such that the regret incurred by any learner $\mathcal{L}$ with \emph{corrupted reward feedback} is no less than $\Omega(dT^{\rho})$. The formulation of such a corruption strategy hinges on the observation that the regret incurred by $\mathcal{L}$ is bounded below by the sum of the Kullback-Leibler (KL) divergence between the distribution of the \emph{corrupted reward feedback} conditioned on different possible values of $\theta$. Specifically, let $\theta$ be uniformly drawn from $\{-\beta, \beta\}^d$. Given an action $a_t$, conditioned on $\theta_i > 0$, the corrupted reward feedback $\hat v_t$ is
\begin{align}\label{1}
    \hat v_t = \mu_{\theta}(a_t) + c_t(a_t|\theta_i > 0) + \xi_{a_t} =  \underbrace{\left(-\frac{1}{2}\|a_t\|^2 + \sum_{j\neq i} \theta_j a_{t, j}\right) + \beta a_{t, i} + c_t(a_t|\theta_i > 0)}_{\textcolor{red}{\mu_1}} + \xi_{a_t}.
\end{align}
Conditioned on $\theta_i < 0$, the corrupted reward feedback is
\begin{align}\label{2}
    \hat v'_t = \mu_{\theta}(a_t) + c_t(a_t|\theta_i < 0) + \xi_{a_t} = \underbrace{\left(-\frac{1}{2}\|a_t\|^2 + \sum_{j\neq i} \theta_j a_{t, j}\right) - \beta a_{t, i} + c_t(a_t| \theta_i < 0)}_{\textcolor{red}{\mu_2}} + \xi_{a_t}.
\end{align}
Consider the following corruption strategy which sets $c_t(a_t|\theta_i > 0) = -\beta a_{t, i}$ and $c_t(a_t) = \beta a_{t, i}$ to minimizes the KL divergence between $\hat v_t$ and $\hat v'_t$. Together with $1$-strongly concavity of $\mu_{\theta}$, we can establish
\begin{equation}\label{eq1}
    \bE\left\{\sum^T_{t=1}\mu_{\theta}(a^*)-\mu_{\theta}(a_t) \right\} \geq \frac{1}{2}\max\left\{\sum^T_{t=1}(\frac{C_\kappa T^{\rho-1}}{\beta} - \beta)^2, \frac{dT\beta^2}{2}\right\}.
\end{equation}
Since $d \leq \frac{1}{C_{\kappa}}T^{1- \rho}$, we can set $\beta = \sqrt{C_\kappa} T^{\frac{\rho-1}{2}}$ to satisfy $\|\theta\|_2 \leq 1$ and to optimize the lower bound in Equation \eqref{eq1}. Then we obtain $\bE\left\{\sum^T_{t=1}\mu_{\theta}(a^*)-\mu_{\theta}(a_t)\right\} \geq dC_{\kappa}T^{\rho}/4$. Notice that the corruption level each round is bounded by $\beta \|a_{t}\|_{\infty}$. In the scenario when the radius of the \emph{action} space $\cA$ is upper bounded by $\beta$, the corruption budget each round is bounded by $C_{\kappa}t^{\rho-1}$. It implies that the corruption is induced by $\rho$-\emph{imperfect} user, completing the proof.
\end{proof} 


 


==> 3-upper-bound.tex <==
\section{The Efficiency-Robustness Tradeoff in LIHF}
Section \ref{sec:lower-bound} shows that a lower bound regret of $\Omega(d\max\{\sqrt{T}, T^{\rho}\})$ is intrinsic for learning from $\rho$-imperfect user, even with known $\rho$. In this section, we study what would be possible --- but in a significantly more challenging learning setting with \emph{arbitrary} and \emph{agnostic} corruption. The reason for fighting for such generality is due to practical considerations; in reality, it is rarely possible to truly predict users' irrationality or behaviors. Technique-wise, gradient-based methods are the most commonly used for addressing continuous action spaces, and so are our approaches. The key novelty in our results is not about the development of fundamentally new algorithmic techniques, but rather the conduct of more fine-grained analysis about two popular gradient-based methods --- Dueling Bandit Gradient Descent (DBGD \citep{Yue2009InteractivelyOI}) and Noisy Comparison-based Stochastic Mirror Descent (NC-SMD) \citep{kumagai2017regret} --- and the proof of how these algorithms can be ``tailored'' to achieve robustness against corruption. On a conceptual level, our key insight is that one can carefully tune the learning rates of these gradient-based methods to gracefully trade off learning efficiency for adversarial robustness --- a interesting concept which we coin the \emph{efficiency-robustness tradeoff}. Notably, en route developing our result, we also pin down a tight lower bound of $\Omega(T^{3/4})$ for the well-known DBGD algorithm which surprisingly remained an open question to date despite extensive studies of this algorithm. 

Our finding reveals the intrinsic tradeoff between robustness and efficiency for gradient-based algorithms under agnostic corruption (Theorem \ref{theorem:regret_upper_bound_DBGD}). In general, the tradeoff is controlled by the exploration size in Algorithm \ref{algo:DBGD} (depends on $\alpha$) (experimentally verified at Appendix \ref{sec:tradeoff}). A higher tolerance of agnostic corruption comes at a cost of worse regret in scenario without corruption, shown by Figure \ref{fig:tradeoff}.

\begin{algorithm}[H]\label{algo:DBGD}
\caption{Dueling Bandit Gradient Descent (DBGD)}
\SetKwInput{KwInput}{Input}
\SetKwInOut{KwOutput}{Output}
\KwInput{Exploration rate $\delta$, exploitation rate $\gamma$,  initial action $a_1 = \mathbf{0} \in \cA$.}
\For{$t \in [T]$}
{
    Sample unit vector $u_t$ uniformly and set $a'_t := \cP_{\cA}\left(a_t + \delta u_t\right)$.\\
    Present action pair $(a_t, a'_t)$ to user and receive corrupted dueling feedback $\hat \cF(a'_t, a_t)$.\\
    Compute gradient $\hat g_t := -\frac{d}{\delta}\hat \cF(a'_t, a_t) u_t$.\\
    Set step size $\eta := \frac{\gamma \delta}{d}$ and update $a_{t+1} := \cP_\cA(a_t - \eta \hat g_t)$.
}
\end{algorithm}

\begin{theorem}[Efficiency-Robustness Tradeoff in DBGD]\label{theorem:regret_upper_bound_DBGD}
For any $ \alpha \in (0,\frac{1}{4}]$ and any number of round $T$ satisfying $T > \left(\frac{\sqrt{2Rd}L_\mu L_2}{\sqrt{13L}L_{\sigma}}\right)^4$, Algorithm \ref{algo:DBGD} parameterized with  $\gamma = \frac{R}{\sqrt{T}}$ and $\delta = \frac{\sqrt{2Rd}}{\sqrt{13 L}T^{\alpha}} $ achieves $\text{Reg}_T \leq O(\sqrt{d}T^{1 - \alpha}+ \sqrt{d}T^{\alpha}C)$ for any total corruption level $C$. 
\end{theorem}

At the core of this proof is a novel development of a  regret decomposition lemma (Lemma \ref{lemma:decomposition_dbgd}), where we decompose the regret into two parts: regret of decision making under uncertainty and regret due to feedback imperfection. This decomposition has been proven to be useful for controlling regret of interactive decision-making in reinforcement learning  \cite{foster2023statistical}. However, to the best of our knowledge,  Lemma \ref{lemma:decomposition_dbgd} is the first to exhibit such a decomposition for dueling feedback, which contains much sparser information than the direct reward feedback as in RL or classic online learning in the aforementioned studies. Hence we believe the lemma may be of independent interest for future research on dueling bandits under corruption or erroneous observation. Our proof employs new techniques and is also more involved. %\hf{Can we say anything about which part of previous proofs do not work under dueling feedback? Or what additional steps you did? I feel like the description is a bit too general that it is not clear what is truly special...for example, does \cite{foster2023statistical} also follow exactly what you are doing below, and if so what's your new part? We really need to emphasize what is \textbf{thing you did but they did not} } 
Previous proofs of the decomposition lemma for  reward feedback crucially hinges on an online estimation oracle \cite{foster2023statistical},  which however cannot be constructed in our problem with dueling feedback with agnostic corruption. We thus have to develop new proof ideas tailored specifically for dueling bandit feedback. We start from  quantifying the bias  $b_t$  caused by adversarial corruption in gradient estimation, and then show that we can control the cumulative impact of bias  by the exploration size $\delta$, i.e. $\sum^T_{t=1}\bE\left(b_t^{\top}(a_t - a^*)\right) \leq  2R dL_{\sigma}C/\delta$. Consequently, 
Lemma \ref{lemma:decomposition_dbgd} shows that the regret of decision and observation error are jointly controlled by the exploration size $\delta$. We choose $\delta$ in order of $\Theta(T^{-\alpha}), \alpha \in (0, 1/4]$ to achieve a balance between optimizing the learning objective \eqref{def:DB_reg} and controlling the gradient bias arising from the \emph{corrupted dueling feedback}. Following this, we show $\text{Reg}_T$ is upper bounded by $O(\sqrt{d}T^{1-\alpha}+ \sqrt{d}T^{\alpha}C)$.

\begin{wrapfigure}{r}{0pt}
    \centering
    \includegraphics[width=0.5\textwidth]{images/tradeoff.pdf}
    \caption{Efficiency-Robustness Tradeoff}
    \label{fig:tradeoff}
\end{wrapfigure}

\begin{lemma}[Regret Decomposition]\label{lemma:decomposition_dbgd} Let $b_t := \frac{d}{\delta}\left(\hat \bP(a'_t \succ a_t) - \bP(a'_t \succ a_t)\right)u_t, u_t \sim \bS$, and choose $\lambda = \frac{L_{\sigma}}{L_{\sigma} - \delta L_{\mu}L_\sigma}$, we have
    \begin{align*} 
        \text{Reg}_T & \leq \underbrace{\lambda\left(\frac{R^2d}{\gamma \delta} + \frac{T \gamma d}{\delta}+ 13\delta LT\right)}_{\textcolor{red}{Regret \hspace{1mm} of \hspace{1mm} Decision}} + \underbrace{2 \lambda \sum^T_{t=1}\bE\left(b_t^{\top}(a_t - a^*)\right)}_{\textcolor{red}{Observation \hspace{1mm} Error}}.
    \end{align*}
\end{lemma}

Note that Algorithm \ref{algo:DBGD} works for general concave user utility. However, if the user displays a strongly concave utility, we can tune learning rate of NC-SMD to get better tradeoff. Specifically, we can get better regret upper bound $\Tilde{O}(d\sqrt{T})$ in scenario without corruption at the same time affording $O(T^{3/4})$ agnostic corruption (see Prop \ref{theorem:regret_upper_bound_unknown}). The proof of Proposition \ref{theorem:regret_upper_bound_unknown} shares similar structure as the proof Theorem \ref{theorem:regret_upper_bound_DBGD}, however working with a different algorithm. We direct readers to Appendix \ref{proof:theorem:regret_upper_bound_DBGD} and \ref{proof:theorem:regret_upper_bound_unknown} to see full statement of Theorem \ref{theorem:regret_upper_bound_unknown}, details of the Algorithm NC-SMD and proof of Proposition \ref{theorem:regret_upper_bound_unknown}.


\begin{proposition}[Efficiency-Robustness Tradeoff in NC-SMD]\label{theorem:regret_upper_bound_unknown}
For any $\alpha \in [\frac{1}{2}, 1)$, if the utility function is strongly concave, by choosing learning rate $\eta = \frac{\sqrt{\log T}}{2d}T^{-\alpha}$, for the Algorithm NC-SMD, we have $\text{Reg}_T \leq \Tilde{O}(dT^{\alpha} + \sqrt{d}T^{\frac{1}{2}(1 - \alpha)}C + dC)$ for any total corruption level $C$.
\end{proposition}

\begin{wrapfigure}{r}{0pt}
    \centering
    \includegraphics[width=0.5\textwidth]{images/lb.pdf}
    \caption{DBGD Lower Bound}
    \label{fig:lb}
\end{wrapfigure}

An interesting corollary of Theorem \ref{theorem:regret_upper_bound_DBGD} is that we can use it to show the DBGD upper bound proved in \citep{Yue2009InteractivelyOI} is tight, which to the best of our knowledge, has not been realized in the previous literature. In the following we provide a sketch of Corollary \ref{theorem:_DBGD_lower_bound}. It has been verified by experiments (see Figure \ref{fig:lb}, simulation details in Appendix \ref{sec:lower_bound_simulation}). We direct readers to Appendix \ref{proof:theorem:_DBGD_lower_bound} for proof details. 


\begin{corollary}[Minimax Lower Bound for DBGD] \label{theorem:_DBGD_lower_bound}
There exists a linear utility function $\mu$ and a link function $\sigma$ such that choosing $\alpha = 1/4$, $\text{Reg}_T$ suffered by Algorithm \ref{algo:DBGD} is at least $\Omega\left(T^{3/4}\right)$.
\end{corollary}

\begin{proof}
\textbf{(Proof Sketch of Corollary \ref{theorem:_DBGD_lower_bound}).} Corollary \ref{theorem:_DBGD_lower_bound} shows that the standard DBGD algorithm with $\alpha = \frac{1}{4}$ can afford $O(T^{3/4})$ agnostic corruption. Moreover, we observe that we can make the sub-optimal arm and the optimal arm indistinguishable by using the total corruption level in the same order of the number of times sub-optimal arm that has been pulled. Therefore, there must exist an problem instance such that the sub-optimal arm has been pulled at least $\Theta(T^{3/4})$ times by DBGD. If not, we can create the parallel world to make DBGD suffer linear regret in one of the environments by using total corruption level less than $\Theta(T^{3/4})$, which contradicts Theorem \ref{theorem:regret_upper_bound_DBGD}. Intuitively, it says that if an environment is "easy" to attack, the agnostic corruption level which an algorithm could afford can not exceed the worst possible regret suffered by the algorithm in scenario without corruption. 
\end{proof}








==> 4-experiment.tex <==
\section{Experiments}
In this section, we study the empirical performance of DBGD and NC-SMD to validate our theoretical analysis by running simulations on both synthetic datasets and real-world recommendation data in comparison with several baseline algorithms. Experimental details can be found at Appendix \ref{sec:additional_experiments}.

\subsection{Synthetic Data}\label{sec:setup}
\textbf{Experiment Setup.} We consider a standard experiment setup, which adopts a strongly concave utility $\mu_{\theta}(a) := \theta^{\top}a - \frac{1}{2}\|a\|^2_2$, a logistic link function $\sigma(x) = \frac{1}{1 + \exp(-x)}$. We choose $d = 5$, and $T = 10^5$. Our \emph{action} space $\cA$ is a $d$-dimensional ball with radius $R = 10$. The preference parameter $\theta$ is randomly sampled from the surface of $\cA$. In our problem setting, the optimal action $a^*$ is $\theta$ and $\mu_{\theta}(a^*) = 50$. We simulate \emph{agnostic} \emph{arbitrary} corruption for $C = T^{\rho}, \rho \in [0.5, 0.75]$. Specifically, we force the user to submit her least preferred item to the algorithm over the first $C$ rounds (for experiments on corruption induced by $\rho$-\emph{imperfect} user, see Appendix \ref{sec:robustness}). For each value of $\rho$, we repeat the experiments for $5$ times, each under a different seed. We use Doubler and Sparring proposed by \cite{ailon2014reducing} as the baseline algorithms for comparison. We set bandit gradient descent \citep{flaxman2004online} as the black-box bandit algorithm. 

\begin{figure}[H]
    \centering
    \raisebox{0pt}[\dimexpr\height-0.6\baselineskip\relax]{\includegraphics[width=\textwidth]{images/figure1.png}}
    \vspace{-20pt}
    \caption{We show the log-log plot for regret occurred by different algorithms under arbitrary agnostic corruption. For each $\rho$, we present the line plot of average regret over $5$ simulations. The shaded region is the average regret $\pm$ one standard deviation. In addition, we fit the order of the average regret, i.e. $\bE(\text{Reg}_T) = T^{o}$, by least squares using last $1\%$ of data. % \XL{polish the caption and plot?}
    }
    \vspace{-10pt}
    \label{Figure1}
\end{figure}

\vspace{10pt}
\noindent \textbf{Results and Discussion.} Figure \ref{Figure1} shows that standard DBGD ($\alpha = 1/4$) and NC-SMD ($\alpha = 1/2$) are able to tolerate $O(T^{3/4})$ unknown corruption, aligning with the theoretical result. Experimentally, NC-SMD enjoys the best performance under strongly concave utility. Empirically, Sparring has comparable performance as DBGD, even though it is a heuristic approach with no theoretical guarantee. The worst performance of Doubler might be attributed to the fact that its theoretical guarantee is only applicable to linear link function, which is different from our experiment setup.%\XL{extend a little bit, about the your finding and analysis that underneath the result.}


\subsection{Spotify Recommendation Data}

\begin{wrapfigure}{r}{0pt}
    \centering
    \raisebox{0pt}[\dimexpr\height-0.6\baselineskip\relax]{\includegraphics[width=0.5\textwidth]{images/figure2.png}}
    \vspace{-10pt}
    \caption{Results on Spotify Recommendation}
    \vspace{-10pt}
    \label{Figure2}
\end{wrapfigure}

\textbf{Evaluation Setup}. We also evaluate our approach on Spotify recommendation data \citep{kaggle}. The objective is to recommend songs to incoming users. This dataset includes $17\times 10^4$ songs ($|\cA| = 17\times 10^4$), each is described by 15 distinct features (d = 15). We create 5 different user types by clustering the dataset into 5 groups. We use the average of the song embedding within each group as the user's preference vector. Our aim is to recommend songs to users that have the highest cosine similarity (utility function) with their preference vectors. We rescale the cosine similarity to $[-100, 100]$. We simulate corruption induced by $\rho$-\emph{imperfect} user to model imperfect human feedback. We only test the performance of DBGD and Sparring because NC-SMD only works under strongly concave utility and Doubler only works under linear link function.

\vspace{10pt}
\noindent \textbf{Results and Discussion.}  Figure \ref{Figure2} show that the performance of DBGD aligns with theoretical prediction on real-world recommendation data, even in the scenario when $\cA$ is discrete and nonconvex. Both DBGD and Sparring are robust to agnostic corruption induced by $\rho$-\emph{imperfect} user, however, empirically it seems that Sparring is invariant to $\rho$. This might because the song embeddings are highly sparse, which results in the fact that the proposed arms according to the heuristic approach are easy to distinguish, even under agnostic corruption.

\vspace{10pt}
\noindent \textbf{Additional Experiments.} We also test the performance of Versatile-DB \citep{pmlr-v162-saha22a}, an approach robust to agnostic corruption with theoretical guarantee. However, this approach is not computationally efficient. When $K = 2000$, running 100 iterations takes around 20 CPU hours and it's performance is dominated by DBGD. We direct readers to Appendix \ref{sec:vdb} to see the details.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\textwidth]{images/figure2.pdf}
%     \caption{Results on Spotify Recommendation Data}
%     \label{Figure2}
% \end{figure}


\section{Conclusion}
In this paper, we model learning from \emph{imperfect} human feedback as a corrupted continuous dueling bandit. We highlight the fundamental difficulty of LIHF by developing a regret lower bound. Then we show that by carefully tuning the learning rates of gradient-based methods, we can gracefully trade off learning efficiency for adversarial robustness. Our theoretical predictions also hold on real-world dataset. For future direction, it is interesting to generalize our setting to include contextual information and design algorithms robust to agnostic corruption. In addition, it is also an interesting open problem to design algorithms performs best-of-both-worlds, i.e. performing optimally both with and without agnostic corruption, in continuous action space.

==> ICLR25/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{tikz}
\usepackage{float}
\usepackage{pdflscape}
\usepackage[ruled, vlined, linesnumbered]{algorithm2e}

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}[section]
\newtheorem*{retheorem}{Theorem}
\newtheorem*{reproposition}{Proposition}
\newtheorem*{relemma}{Lemma}
\newtheorem*{recorollary}{Corollary}
\newtheorem{definition}{Definition}[section]
\newtheorem{assumption}{Assumption}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}[section]
\fi
\ifx\example\undefined
\newtheorem{example}[theorem]{Example}
\fi
\ifx\property\undefined
\newtheorem{property}{Property}
\fi
\ifx\lemma\undefined
\newtheorem{lemma}{Lemma}[section]
\fi
\ifx\proposition\undefined
\newtheorem{proposition}{Proposition}
\fi

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

